On the Impact of the Capacity Drop Phenomenon for Freeway Traffic Flow Control

Capacity drop is an empirically observed phenomenon in vehicular traffic flow on freeways whereby, after a critical density is reached, a state of congestion sets in, but the freeway does not become decongested again until the density drops well below the critical density. This introduces a hysteresis effect so that it is easier to enter the congested state than to leave it. However, many existing first-order models of traffic flow, particularly those used for control design, ignore capacity drop, leading to suboptimal controllers. In this paper, we consider a cell transmission model of traffic flow that incorporates capacity drop to study the problem of optimal freeway ramp metering. We show that, if capacity drop is ignored in the control design, then the resulting controller, obtained via a convex program, may be significantly suboptimal. We then propose an alternative model predictive controller that accounts for capacity drop via a mixed integer linear program and show that, for sufficiently large rollout horizon, this controller is optimal. We also compare these approaches to a heuristic hand-crafted controller that is viewed as a modification of an integral feedback controller to account for capacity drop. This heuristic controller outperforms the controller that ignores capacity drop but underperforms compared to the proposed alternative model predictive controller. These results suggest that it is generally important to include capacity drop in the controller design process, and we demonstrate this insight on several case studies.

==> figures/2cell.tex <==
% This file was created by tikzplotlib v0.9.0.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
title={Cars Exiting Network Per Timestep},
x grid style={white!69.0196078431373!black},
xlabel={Time Step},
xmin=-2.95, xmax=83.95,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Number of Cars Exited},
ymin=36.6761863425926, ymax=80.1230034722222,
ytick style={color=black}
]
\addplot [semithick, color0, dotted]
table {%
1 78.1481481481482
2 55.679012345679
3 48.1893004115226
4 45.6927297668038
5 44.8605395518976
6 44.5831428135955
7 44.4906772341615
8 44.4598553743501
9 44.4495814210796
10 44.4461567699896
11 44.445015219626
12 44.4446347028384
13 44.4445078639091
14 44.444465584266
15 44.4444514910516
16 44.4444467933135
17 44.4444452274008
18 44.44444470543
19 44.4444445314396
20 44.4444444734428
21 44.4444444541106
22 44.4444444476665
23 44.4444444455185
24 44.4444444448025
25 44.4444444445637
26 44.4444444444844
27 44.4444444444578
28 44.4444444444489
29 44.4444444444459
30 44.4444444444448
31 44.4444444444446
32 44.4444444444443
33 44.4444444444443
34 44.4444444444443
35 44.4444444444443
36 44.4444444444443
37 44.4444444444443
38 44.4444444444443
39 44.4444444444443
40 44.4444444444443
41 44.4444444444443
42 44.4444444444443
43 44.4444444444443
44 44.4444444444443
45 44.4444444444441
46 44.4444444444443
47 44.4444444444443
48 44.4444444444443
49 44.4444444444443
50 44.4444444444443
51 44.4444444444443
52 44.4444444444443
53 44.4444444444443
54 44.4444444444443
55 44.4444444444443
56 44.4444444444443
57 44.4444444444443
58 44.4444444444443
59 44.4444444444443
60 44.4444444444443
61 44.4444444444443
62 44.4444444444443
63 44.4444444444443
64 44.4444444444443
65 44.4444444444443
66 44.4444444444443
67 44.4444444444443
68 44.4444444444443
69 44.4444444444443
70 44.4444444444443
71 44.4444444444443
72 44.4444444444443
73 44.4444444444443
74 44.4444444444443
75 44.4444444444443
76 44.4444444444443
77 44.4444444444443
78 44.4444444444443
79 44.4444444444443
80 44.4444444444443
};
\addlegendentry{RAMPC}
\addplot [semithick, color1, dash pattern=on 1pt off 3pt on 3pt off 3pt]
table {%
1 78.1481481481482
2 55.679012345679
3 47.8086419753086
4 43.4166666666667
5 40.875
6 39.6041666666666
7 38.96875
8 38.6510416666666
9 39.5755208333334
10 44.9127604166666
11 50.0188802083333
12 53.7906901041667
13 56.2859700520833
14 57.8382975260417
15 58.7668050130208
16 59.3072306315105
17 59.6155293782551
18 59.7887217203777
19 59.8848393758137
20 59.9376589457195
21 59.9664491017661
22 59.9820343653359
23 59.9904220898948
24 59.9949134985604
25 59.9973079760871
26 59.9985796014466
27 59.9992526074252
28 59.9996077070632
29 59.9997945552072
30 59.9998926284411
31 59.9999439896396
32 59.999970832529
33 59.9999848351194
34 59.9999921269869
35 59.9999959182073
36 59.9999978864603
37 59.9999989069088
38 59.9999994352938
39 59.9999997085661
40 59.9999998497433
41 59.9999999226011
42 59.999999960166
43 59.999999979515
44 59.999999989474
45 59.9999999945949
46 59.999999997227
47 59.9999999985776
48 59.9999999992715
49 59.9999999996267
50 59.999999999809
51 59.9999999999022
52 59.99999999995
53 59.9999999999745
54 59.9999999999868
55 59.9999999999932
56 59.9999999999968
57 59.9999999999982
58 59.9999999999991
59 59.9999999999995
60 60
61 60
62 60
63 60
64 60
65 60
66 60
67 60
68 60
69 60
70 60
71 60
72 60
73 60
74 60
75 60
76 60
77 60
78 60
79 60
80 60
};
\addlegendentry{HC}
\addplot [semithick, color2, dashed]
table {%
1 78.1481481481482
2 55.679012345679
3 48.1893004115226
4 45.6927297668038
5 44.8605395518976
6 44.5831428135955
7 44.4906772341615
8 44.4598553743501
9 44.4495814210796
10 44.4461567699896
11 44.445015219626
12 44.4446347028384
13 44.4445078639091
14 44.444465584266
15 44.4444514910516
16 44.4444467933135
17 44.4444452274008
18 44.44444470543
19 44.4444445314396
20 44.4444444734428
21 44.4444444541106
22 44.4444444476665
23 44.4444444455185
24 44.4444444448025
25 44.4444444445637
26 44.4444444444844
27 44.4444444444578
28 44.4444444444489
29 44.4444444444459
30 44.4444444444448
31 44.4444444444446
32 44.4444444444443
33 44.4444444444443
34 44.4444444444443
35 44.4444444444443
36 44.4444444444443
37 44.4444444444443
38 44.4444444444443
39 44.4444444444443
40 44.4444444444443
41 44.4444444444443
42 44.4444444444443
43 44.4444444444443
44 44.4444444444443
45 44.4444444444441
46 44.4444444444443
47 44.4444444444443
48 44.4444444444443
49 44.4444444444443
50 44.4444444444443
51 44.4444444444443
52 44.4444444444443
53 44.4444444444443
54 44.4444444444443
55 44.4444444444443
56 44.4444444444443
57 44.4444444444443
58 44.4444444444443
59 44.4444444444443
60 44.4444444444443
61 44.4444444444443
62 44.4444444444443
63 44.4444444444443
64 44.4444444444443
65 44.4444444444443
66 44.4444444444443
67 44.4444444444443
68 44.4444444444443
69 44.4444444444443
70 44.4444444444443
71 44.4444444444443
72 44.4444444444443
73 44.4444444444443
74 44.4444444444443
75 44.4444444444443
76 44.4444444444443
77 44.4444444444443
78 44.4444444444443
79 44.4444444444443
80 44.4444444444443
};
\addlegendentry{None}
\addplot [semithick, color3]
table {%
1 78.1481481481482
2 55.679012345679
3 48.1893004115226
4 44.4844855967078
5 39.5890946502058
6 43.4679732510288
7 48.5706995884774
8 52.7037062757202
9 55.5610313786008
10 57.3851048096707
11 58.4948469650207
12 59.1485707626028
13 59.5248590213478
14 59.7377163306969
15 59.8565015753601
16 59.9220724926857
17 59.9579470988458
18 59.9774289756743
19 59.9879422009628
20 59.9935849570443
21 59.9965994068036
22 59.9982031675427
23 59.9990533158416
24 59.9995025239559
25 59.9997391949958
26 59.9998635640065
27 59.9999287652577
28 59.9999628742562
29 59.9999806829414
30 59.9999899643776
31 59.9999947936424
32 59.9999973025476
33 59.9999986041373
34 59.9999992785004
35 59.999999627466
36 59.999999807841
37 59.9999999009742
38 59.9999999490142
39 59.9999999737706
40 59.9999999865172
41 59.9999999930742
42 59.9999999964452
43 59.9999999981765
44 59.999999999065
45 59.9999999995212
46 59.9999999997549
47 59.9999999998745
48 59.9999999999359
49 59.9999999999673
50 59.9999999999832
51 59.9999999999914
52 59.9999999999955
53 59.9999999999977
54 59.9999999999986
55 59.9999999999995
56 59.9999999999995
57 60
58 60
59 60
60 60
61 60
62 60
63 60
64 60
65 60
66 60
67 60
68 60
69 60
70 60
71 60
72 60
73 60
74 60
75 60
76 60
77 60
78 60
79 60
80 60
};
\addlegendentry{EHMPC}
\end{axis}

\end{tikzpicture}


==> figures/3cell.tex <==
% This file was created by tikzplotlib v0.9.0.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
title={Cars Exiting Network Per Time Step},
x grid style={white!69.0196078431373!black},
xlabel={Time Step},
xmin=-2.95, xmax=83.95,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Number of Cars Exited},
ymin=30.1818741793151, ymax=59.4798754799973,
ytick style={color=black}
]
\addplot [semithick, color0, dotted]
table {%
1 58.1481481481481
2 48.8641975308642
3 46.5316872427984
4 45.5098491083676
5 45.0663246456333
6 44.8760132296906
7 44.7955345689173
8 44.7621445272232
9 44.7486458410992
10 44.743388120908
11 44.7414553514855
12 44.7408138090882
13 44.7406446309697
14 44.7406307853475
15 44.7406568761405
16 44.7406853278857
17 44.7407067433875
18 44.7407208062989
19 44.7407294034959
20 44.7407344327739
21 44.7407372883965
22 44.7407388753337
23 44.7407397430609
24 44.7407402115784
25 44.7407404620092
26 44.7407405947713
27 44.7407406646744
28 44.7407407012695
29 44.7407407203341
30 44.7407407302242
31 44.7407407353362
32 44.7407407379703
33 44.7407407393237
34 44.7407407400174
35 44.7407407403721
36 44.7407407405531
37 44.7407407406456
38 44.7407407406922
39 44.7407407407163
40 44.7407407407284
41 44.7407407407343
42 44.7407407407377
43 44.7407407407393
44 44.74074074074
45 44.7407407407404
46 44.7407407407404
47 44.7407407407404
48 44.7407407407404
49 44.7407407407404
50 44.7407407407404
51 44.7407407407404
52 44.7407407407404
53 44.7407407407404
54 44.7407407407404
55 44.7407407407404
56 44.7407407407404
57 44.7407407407404
58 44.7407407407404
59 44.7407407407404
60 44.7407407407404
61 44.7407407407404
62 44.7407407407404
63 44.7407407407404
64 44.7407407407404
65 44.7407407407404
66 44.7407407407404
67 44.7407407407404
68 44.7407407407404
69 44.7407407407404
70 44.7407407407404
71 44.7407407407404
72 44.7407407407404
73 44.7407407407404
74 44.7407407407404
75 44.7407407407404
76 44.7407407407404
77 44.7407407407404
78 44.7407407407404
79 44.7407407407404
80 44.7407407407404
};
\addlegendentry{RAMPC}
\addplot [semithick, color1, dash pattern=on 1pt off 3pt on 3pt off 3pt]
table {%
1 58.1481481481481
2 48.8641975308642
3 46.5316872427984
4 44.5986008230452
5 40.5368641975309
6 37.3579838134431
7 35.2287121079103
8 33.8221829632678
9 32.9023859727582
10 32.3053502793175
11 31.9199788737461
12 31.6722859170214
13 31.5136015111643
14 33.4799534536413
15 39.0117894506806
16 42.486067475143
17 44.6340258618292
18 45.9836484779239
19 46.8384094681172
20 47.3797580952396
21 47.7226122257505
22 47.9397531750741
23 48.0772757763124
24 48.1643734237632
25 48.2195352671488
26 48.2544711012929
27 48.2765971295844
28 48.2906102808354
29 48.2994852766278
30 48.3051061072963
31 48.3086659667199
32 48.3109205443545
33 48.3123484435234
34 48.3132527796636
35 48.3138255258857
36 48.3141882651596
37 48.3144180000331
38 48.3145634987864
39 48.3146556479969
40 48.3147140091635
41 48.3147509712355
42 48.314774380548
43 48.3147892064458
44 48.3147985961812
45 48.3148045430135
46 48.3148083093406
47 48.314810694681
48 48.3148122053967
49 48.3148131621833
50 48.3148137681483
51 48.3148141519259
52 48.3148143949852
53 48.3148145489226
54 48.3148146464164
55 48.3148147081624
56 48.3148147472684
57 48.3148147720353
58 48.3148147877209
59 48.3148147976553
60 48.3148148039472
61 48.3148148079322
62 48.3148148104556
63 48.314814812054
64 48.3148148130663
65 48.3148148137075
66 48.3148148141136
67 48.3148148143705
68 48.3148148145333
69 48.3148148146365
70 48.314814814702
71 48.3148148147434
72 48.3148148147693
73 48.3148148147861
74 48.3148148147966
75 48.3148148148034
76 48.3148148148075
77 48.3148148148102
78 48.3148148148121
79 48.314814814813
80 48.3148148148134
};
\addlegendentry{HC}
\addplot [semithick, color2, dashed]
table {%
1 58.1481481481481
2 48.8641975308642
3 46.5316872427984
4 45.5098491083676
5 44.3704957577605
6 43.4684076817558
7 42.8824523264859
8 42.4715223941924
9 42.1651850092602
10 41.9267524936292
11 41.7359214285603
12 41.5805648000494
13 41.4528132638455
14 41.3471527334234
15 41.259475196843
16 41.1865846055637
17 41.1259236566817
18 41.0754107641884
19 41.0333343729566
20 40.9982789669917
21 40.9690699802718
22 40.9447309554113
23 40.9244492734836
24 40.9075482633122
25 40.8934642708391
26 40.8817276956906
27 40.8719472561818
28 40.8637969084891
29 40.857004960742
30 40.851345008329
31 40.8466283832047
32 40.8426978631487
33 40.8394224301792
34 40.8366929028966
35 40.8344182969172
36 40.8325227919759
37 40.8309432045448
38 40.8296268816939
39 40.8285299459899
40 40.8276158329047
41 40.8268540720012
42 40.8262192712491
43 40.8256902706225
44 40.8252494367669
45 40.8248820752206
46 40.8245759405988
47 40.8243208284141
48 40.8241082349266
49 40.8239310736869
50 40.8237834393203
51 40.8236604106819
52 40.8235578868166
53 40.8234724502622
54 40.8234012531334
55 40.8233419221924
56 40.8232924797421
57 40.8232512776999
58 40.8232169426647
59 40.8231883301355
60 40.8231644863613
61 40.8231446165491
62 40.8231280583727
63 40.823114259892
64 40.8231027611582
65 40.8230931788803
66 40.8230851936482
67 40.8230785392884
68 40.8230729939887
69 40.8230683729053
70 40.8230645220028
71 40.8230613129172
72 40.8230586386794
73 40.8230564101477
74 40.8230545530378
75 40.8230530054466
76 40.8230517157872
77 40.8230506410705
78 40.8230497454738
79 40.8230489991429
80 40.8230483772008
};
\addlegendentry{None}
\addplot [semithick, color3]
table {%
1 58.1481481481481
2 48.8641975308642
3 44.5316872427984
4 42.1108631814256
5 35.9850566478688
6 33.0937647208251
7 38.8856732611899
8 45.9296446832293
9 48.7298739394402
10 48.7703073400904
11 48.7905240404156
12 48.8006323905782
13 48.8056865656595
14 48.8082136532
15 48.8094771969704
16 48.8101089688556
17 48.8104248547982
18 48.8105827977694
19 48.810661769255
20 48.8107012549979
21 48.8107209978693
22 48.810730869305
23 48.8107358050229
24 48.810738272882
25 48.8107395068114
26 48.810740123776
27 48.8107404322584
28 48.8107405864996
29 48.8107406636202
30 48.8107407021803
31 48.8107407214607
32 48.8107407311009
33 48.8107407359207
34 48.8107407383309
35 48.8107407395357
36 48.8107407401383
37 48.8107407404395
38 48.8107407405903
39 48.8107407406656
40 48.8107407407031
41 48.8107407407219
42 48.8107407407315
43 48.8107407407358
44 48.8107407407383
45 48.8107407407401
46 48.8107407407415
47 48.8107407407415
48 48.8107407407415
49 48.8107407407415
50 48.8107407407415
51 48.810740740741
52 48.8107407407292
53 48.8107407407015
54 48.8107407407124
55 48.8107407407169
56 48.8107407407392
57 48.8107407407465
58 48.8107407407479
59 48.810740740747
60 48.8107407407451
61 48.8107407407442
62 48.8107407407429
63 48.8107407407406
64 48.8107407407406
65 48.8107407407406
66 48.8107407407406
67 48.8107407407406
68 48.8107407407406
69 48.8107407407406
70 48.8107407407406
71 48.8107407407406
72 48.8107407407406
73 48.8107407407406
74 48.8107407407406
75 48.8107407407406
76 48.8107407407406
77 48.8107407407406
78 48.8107407407406
79 48.8107407407406
80 48.8107407407406
};
\addlegendentry{EHMPC}
\end{axis}

\end{tikzpicture}


==> figures/8cell.tex <==
% This file was created by tikzplotlib v0.9.0.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
title={Eight cell system},
x grid style={white!69.0196078431373!black},
xlabel={Time Step},
xmin=-3.05, xmax=86.05,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ymin=41.8148226149993, ymax=99.6666662952293,
ytick style={color=black},
width=4cm,
height=5cm
]
\addplot [semithick, color0, dotted]
table {%
1 97.037037037037
2 74.9176954732511
3 67.9334959101763
4 65.9941484567431
5 65.7360825462177
6 66.037962246074
7 66.5258578857771
8 67.0501139930319
9 67.508474550143
10 67.9701283898665
11 68.430102565052
12 68.883063956099
13 69.1497741174454
14 69.4265935598138
15 69.6881446053681
16 69.9249966400962
17 69.9488053736932
18 69.9519074294201
19 69.835820994992
20 69.7971255168491
21 69.7842270241349
22 69.7799275265636
23 69.7784943607062
24 69.7780166387538
25 69.7778573981032
26 69.7778043178864
27 69.7777866244805
28 69.7777807266787
29 69.7777787607449
30 69.7777781054335
31 69.7777778869963
32 69.777777814184
33 69.7777777899128
34 69.7777777818233
35 69.7777777791262
36 69.7777777782262
37 69.7777777779279
38 69.7777777778274
39 69.7777777777942
40 69.7777777777828
41 69.7777777777796
42 69.7777777777783
43 69.7777777777778
44 69.7777777777774
45 69.7777777777774
46 69.7777777777774
47 69.7777777777774
48 69.7777777777774
49 69.7777777777774
50 69.7777777777774
51 69.7777777777774
52 69.7777777777774
53 69.7777777777774
54 69.7777777777774
55 69.7777777777774
56 69.7777777777774
57 69.7777777777774
58 69.7777777777774
59 69.7777777777774
60 69.7777777777774
61 69.7777777777774
62 69.7777777777774
63 69.7777777777774
64 69.7777777777774
65 69.7777777777774
66 69.7777777777774
67 69.7777777777774
68 69.7777777777774
69 69.7777777777774
70 69.7777777777774
71 69.7777777777774
72 69.7777777777774
73 69.7777777777774
74 69.7777777777774
75 69.7777777777774
76 69.7777777777774
77 69.7777777777774
78 69.7777777777774
79 69.7777777777774
80 69.7777777777774
81 69.7777777777774
82 69.7777777777774
};
\addlegendentry{RAMPC}
\addplot [semithick, color1, dash pattern=on 1pt off 3pt on 3pt off 3pt]
table {%
1 97.037037037037
2 74.9176954732511
3 67.9334959101763
4 65.9941484567431
5 65.7360825462177
6 66.037962246074
7 66.5258578857771
8 67.0078591432267
9 67.0104377005872
10 66.158237167015
11 65.5379269352522
12 65.0665845441091
13 64.6973155358295
14 63.8813191876443
15 63.4254839236769
16 65.3863516583949
17 74.8843281844295
18 79.2415165418181
19 81.2348324807754
20 82.1506455836304
21 82.5944900581133
22 83.8880272312338
23 84.6336076532864
24 84.0294770700075
25 83.8389098826156
26 83.6737530040621
27 83.5112291779096
28 83.3668622843568
29 83.2510369414763
30 83.1648225670956
31 85.9514704253506
32 86.412911564817
33 86.3862242435798
34 86.3863289691685
35 86.385286085082
36 86.3838519373044
37 86.3823742753029
38 86.3810016208754
39 86.3797871074726
40 86.3787396956131
41 86.3778491937196
42 86.3770982794686
43 86.3764681029238
44 86.3759407484677
45 86.3755001827535
46 86.3751324928248
47 86.3748258086339
48 86.3745701005168
49 86.3743569414396
50 86.3741792743858
51 86.3740312012628
52 86.3739077983714
53 86.3738049583162
54 86.3737192561157
55 86.3736478365363
56 86.3735883196823
57 86.373538722034
58 86.3734973905266
59 86.3734629475357
60 86.3734342450107
61 86.3734103262213
62 86.3733903938892
63 86.3733737836083
64 86.3733599417046
65 86.3733484067852
66 86.3733387943512
67 86.3733307839893
68 86.3733241086875
69 86.3733185459359
70 86.3733139103097
71 86.3733100472882
72 86.3733068281026
73 86.3733041454489
74 86.3733019099036
75 86.3733000469492
76 86.3732984944872
77 86.3732972007692
78 86.3732961226706
79 86.3732952242553
80 86.3732944755757
81 86.373293851676
82 86.3732933317597
};
\addlegendentry{HC}
\addplot [semithick, color2, dashed]
table {%
1 97.037037037037
2 74.9176954732511
3 64.600162576843
4 59.2657533950147
5 55.5878581901744
6 52.7194570496761
7 51.0885974978672
8 49.8342282013887
9 48.9282254436119
10 48.1783601220998
11 47.555184679718
12 47.0364425862482
13 46.6043477667506
14 46.2443321699673
15 45.9443403124693
16 45.6943541444949
17 45.4860346867188
18 45.3124359215282
19 45.1677705448546
20 45.0472161512889
21 44.9467541856488
22 44.863035890615
23 44.7932706479755
24 44.7351329468502
25 44.6866848629368
26 44.646311459795
27 44.6126669572168
28 44.5846298717483
29 44.5612656338621
30 44.5417954356249
31 44.525570270428
32 44.5120492994304
33 44.5007818235995
34 44.4913922604071
35 44.4835676244131
36 44.4770470944184
37 44.4716133194227
38 44.4670851735927
39 44.463311718735
40 44.4601671730197
41 44.4575467182572
42 44.4553630059552
43 44.4535432457033
44 44.4520267788266
45 44.4507630564299
46 44.4497099544319
47 44.4488323694341
48 44.4481010486029
49 44.4474916145759
50 44.4469837528877
51 44.4465605348137
52 44.4462078530855
53 44.4459139516448
54 44.4456690337784
55 44.4454649355557
56 44.4452948537041
57 44.4451531188274
58 44.4450350064303
59 44.4449365794326
60 44.4448545569344
61 44.4447862048528
62 44.4447292447849
63 44.4446817780613
64 44.4446422224587
65 44.4446092594562
66 44.4445817902874
67 44.4445588993135
68 44.4445398235021
69 44.4445239269921
70 44.4445106799012
71 44.4444996406583
72 44.4444904412894
73 44.4444827751486
74 44.4444763866982
75 44.4444710629891
76 44.4444666265649
77 44.4444629295444
78 44.4444598486948
79 44.4444572813195
80 44.4444551418405
81 44.4444533589412
82 44.4444518731916
};
\addlegendentry{None}
\addplot [semithick, color3]
table {%
1 97.037037037037
2 74.9176954732511
3 67.9334959101763
4 65.9941484567431
5 65.7360825462177
6 66.037962246074
7 66.5258578857771
8 67.0501139930319
9 67.508474550143
10 67.836299883811
11 67.2570341993257
12 66.2732237957721
13 65.6365235824917
14 63.6760737121697
15 65.2408601792426
16 78.1718281835713
17 85.049935303279
18 85.2321014893043
19 85.4424511478921
20 85.6564776336277
21 85.8059588244928
22 85.8908759702963
23 85.7592603544608
24 85.3456937698518
25 84.3081684585311
26 83.7011335623361
27 84.4546692926538
28 85.2689312782495
29 86.3965707428811
30 86.0900009289762
31 85.6598193323712
32 86.008270698956
33 86.2938912765203
34 86.3247833860291
35 86.3238662650806
36 86.3229258657243
37 86.3220834889621
38 86.3213619381158
39 86.3207541223405
40 86.3202454347256
41 86.3198208035574
42 86.3194667026432
43 86.3191715380131
44 86.3189255406419
45 86.3187205338841
46 86.3185496919368
47 86.318407322653
48 86.3182886812519
49 86.3181898133071
50 86.3181074233162
51 86.3180387649782
52 86.3179815496924
53 86.3179338702857
54 86.3178941374472
55 86.3178610267487
56 86.3178334344984
57 86.3178104409571
58 86.3177912796727
59 86.3177753119362
60 86.3177620054885
61 86.3177509167826
62 86.3177416761937
63 86.317733975704
64 86.3177275586286
65 86.3177222110653
66 86.3177177547632
67 86.3177140411781
68 86.3177109465232
69 86.3177083676446
70 86.3177062185796
71 86.3177044276908
72 86.3177029352846
73 86.3177016916125
74 86.3177006552187
75 86.317699791558
76 86.3176990718403
77 86.3176984720749
78 86.3176979722712
79 86.3176975557681
80 86.3176972086821
81 86.3176969194437
82 86.3176966784113
};
\addlegendentry{EHMPC}
\end{axis}

\end{tikzpicture}


==> figures/horizon_results.tex <==
% This file was created by tikzplotlib v0.9.0.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0, 0, 0}
\definecolor{color1}{rgb}{0, 0, 0}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.03,0.97)}, anchor=north west, draw=white!80!black},
tick align=outside,
tick pos=left,
title={Total Outflow vs. Horizon Length},
x grid style={white!69.0196078431373!black},
xlabel={Horizon Length},
xmin=0.254770340140478, xmax=14.7452296598595,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Total Car Outflow},
ymin=3534.21816184757, ymax=4878.02036709351,
ytick style={color=black}
]
\addplot[only marks, mark=+, draw=color0, fill=color0, colormap/viridis]
table{%
x                      y
1 3606.11111111111
2 3606.11111111111
3 3606.11111111111
4 3606.11111111111
5 3606.11111111111
6 4768.76741455189
7 4816.93033179012
8 4816.93033179012
9 4816.93033179012
10 4816.93033179012
11 4816.93033179012
12 4816.93033179012
13 4816.93033179012
14 4816.93033179012
};
\addlegendentry{[110, 70]}
\addplot [only marks, mark=o, draw=color1, fill=color1, colormap/viridis]
table{%
x                      y
1 3606.11111111111
2 3606.11111111111
3 3606.11111111111
4 3606.11111111111
5 3606.11111111111
6 3606.11111111111
7 3606.11111111111
8 3606.11111111111
9 3606.11111111111
10 4212.53989690513
11 4399.52701388888
12 4399.52701388888
13 4399.52701388888
14 4399.52701388888
};
\addlegendentry{[100, 60]}
\end{axis}

\end{tikzpicture}

